A Practical Introduction to Benchmarking and Characterization of Quantum Computers

Rapid progress in quantum technology has transformed quantum computing and quantum information science from theoretical possibilities into tangible engineering challenges. Breakthroughs in quantum algorithms, quantum simulations, and quantum error correction are bringing useful quantum computation closer to fruition. These remarkable achievements have been facilitated by advances in quantum characterization, verification, and validation (QCVV). QCVV methods and protocols enable scientists and engineers to scrutinize, understand, and enhance the performance of quantum information-processing devices. In this tutorial, we review the fundamental principles underpinning QCVV, and introduce a diverse array of QCVV tools used by quantum researchers. We define and explain QCVV's core models and concepts -- quantum states, measurements, and processes -- and illustrate how these building blocks are leveraged to examine a target system or operation. We survey and introduce protocols ranging from simple qubit characterization to advanced benchmarking methods. Along the way, we provide illustrated examples and detailed descriptions of the protocols, highlight the advantages and disadvantages of each, and discuss their potential scalability to future large-scale quantum computers. This tutorial serves as a guidebook for researchers unfamiliar with the benchmarking and characterization of quantum computers, and also as a detailed reference for experienced practitioners.

==> Tables/be_gc.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}

\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c | c | l}
    \hline
    \hline
    Mathematical & Graphical & Description \\
    \hline
    $\ket{\psi}$ & \includegraphics[height=0.75cm]{Figures/ket.pdf} & State vector (ket) \\
    $\bra{\psi}$ & \includegraphics[height=0.75cm]{Figures/bra.pdf} & Dual vector (bra) \\
    $\sum_i \ketbra{i}{i}$ & \includegraphics[height=0.75cm]{Figures/summation.pdf} & Summation \\
    $\rho$       & \includegraphics[height=0.75cm]{Figures/operator.pdf} & Linear (e.g., density) operator \\
    \hline
    \hline
\end{tabular}}
\caption{
\textbf{Basic Elements of Graphical Calculus.}
A state vector (i.e., ket $\ket{\psi}$) is represented by a wire leading into a triangle from left to right (opposite the direction of quantum circuits). Each wire represents the dimension $d$ of the system, thus one can represent higher-dimensional systems by adding more wires. 
A dual vector (i.e., bra $\bra{\psi}$) is represented by a triangle with a wire leading away from it.
Summation is denoted by coloring the elements being summed over.
And a linear operator, such as a density matrix $\rho$, is represented by a box with wires on both sides.
}
\label{tab:basic_elements}

\end{table}


==> Tables/hc_gc.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}

\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{c | c | l}
    \hline
    \hline
    Mathematical & Graphical & Description \\
    \hline
    $\ket{\psi}^\dagger = \bra{\psi}$ & \includegraphics[height=1.25cm]{Figures/ket_hc.pdf} & Conjugate transpose of a ket \\
    $\bra{\psi}^\dagger = \ket{\psi}$ & \includegraphics[height=1.25cm]{Figures/bra_hc.pdf} & Conjugate transpose of a bra \\
    $\rho^\dagger$                    & \includegraphics[height=1.25cm]{Figures/operator_hc.pdf} & Conjugate transpose of an operator \\
    \hline
    \hline
\end{tabular}}
\caption{
\textbf{Complex Conjugation and Transposition.} 
The complex conjugate of $\psi$ and $\rho$ is denoted $\bar{\psi}$ and $\bar{\rho}$. The transposition of vectors and operators is denoted as a \emph{bending} of the wires leading to and/or from the graphical object. Together, they represented the conjugate transpose 
}
\label{tab:conjugate_tranpose}

\end{table*}


==> Tables/math_gc.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}

\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c | c | l}
    \hline
    \hline
    Mathematical & Graphical & Description \\
    \hline
    $\Tr(\rho)$ & \includegraphics[height=1.05cm]{Figures/matrix_trace.pdf} & Trace of a matrix \\
    $\rho \otimes \sigma$ & \includegraphics[height=1.5cm]{Figures/operator_tensor.pdf} & Tensor product of matrices \\
    $\rho \cdot \sigma$ & \includegraphics[height=0.75cm]{Figures/operator_multiply.pdf} & Matrix multiplication \\
    $\sket{\rho}$ & \includegraphics[height=0.8cm]{Figures/vectorization.pdf} & Vectorization \\
    $M_{ij} = \bra{i}M\ket{j}$ & \includegraphics[height=0.75cm]{Figures/matrix_elements.pdf} & Matrix elements \\
    \hline
    \hline
\end{tabular}}
\caption{
\textbf{Mathematics of Operators.}
The trace of an operator is depicted by connecting the wires leading to/from the operators.
The tensor product of two (or more) operators (e.g., $\rho \otimes \sigma$) is depicted by their vertical alignment along different wires.
The matrix multiplication of two (or more) operators (e.g., $\rho \cdot \sigma$) is depicted by their horizontal alignment along the same wire.
The vectorization of an operator (\eq\ref{eq:vectorization}) is depicted as a graphical ket with two wires leading to it.
And the elements of a matrix $M$ are denoted by an operator surrounded by a bra and a ket.
}
\label{tab:math_op}

\end{table}

